Temporal Action Proposal Generation with Transformers

Transformer networks are effective at modeling long-range contextual information and have recently demonstrated exemplary performance in the natural language processing domain. Conventionally, the temporal action proposal generation (TAPG) task is divided into two main sub-tasks: boundary prediction and proposal confidence prediction, which rely on the frame-level dependencies and proposal-level relationships separately. To capture the dependencies at different levels of granularity, this paper intuitively presents a unified temporal action proposal generation framework with original Transformers, called TAPG Transformer, which consists of a Boundary Transformer and a Proposal Transformer. Specifically, the Boundary Transformer captures long-term temporal dependencies to predict precise boundary information and the Proposal Transformer learns the rich inter-proposal relationships for reliable confidence evaluation. Extensive experiments are conducted on two popular benchmarks: ActivityNet-1.3 and THUMOS14, and the results demonstrate that TAPG Transformer outperforms state-of-the-art methods. Equipped with the existing action classifier, our method achieves remarkable performance on the temporal action localization task. Codes and models will be available.

==> table_tex/ablation_layers.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{cccccc}
\hline

N  &0.3 &0.4 &0.5 &0.6&0.7 \\ \hline
1 & 64.8 & 59.0 & 50.5 & 40.0& 27.9 \\
3 & \textbf{65.3} & \textbf{59.3} & \textbf{50.8} & \textbf{40.1}& \textbf{28.5} \\
6 & 64.2 & 57.6 & 49.2 & 38.9& 26.4 \\
\hline
\end{tabular}
}

\caption{Ablation experiments in the test set of THUMOS14.Performance evaluation on Transformers different layers number.}
\label{ablation_layers}
\end{table}


==> table_tex/ablation_module.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{ccccccc}
\hline

Model & Module  &0.3 &0.4 &0.5 &0.6&0.7 \\ \hline
BMN & TEM & 41.9 &36.4 & 27.8 & 21.6& 12.7 \\
BMN & TEM+PEM & 56.0 & 47.4 & 38.8 & 29.7& 20.5 \\ \hline
TAG Transformer & BTR & 43.8 & 37.7 & 29.9 & 20.8& 12.9\\
TAG Transformer & BTR + PEM& 60.6 & 54.5 & 46.3 & 37.6& 27.1\\
TAG Transformer & TEM + PTR & 62.9 & 57.6 & 47.6 & 37.5& 25.3\\
TAG Transformer & BTR + PTR & \textbf{65.3} & \textbf{59.3} & \textbf{50.8} & \textbf{40.1}& \textbf{28.5}\\
\hline
\end{tabular}
}

\caption{Ablation experiments in the test set of THUMOS14.Performance evaluation on different components of our TAGP Transformers and BMN.  }
\label{ablation module}
\end{table}


==> table_tex/ablation_query.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{cccccc}
\hline

Query  &0.3 &0.4 &0.5 &0.6&0.7 \\ \hline
Learnable parameters & 62.1 & 54.1 & 45.8 & 34.8 & 23.2 \\
Encoder output & 64.2 & 57.4 & 48.7 & 39.1 & 26.8 \\
Original Feature & 65.3 & 59.3 & 50.8 & 40.1 & 28.5 \\
\hline
\end{tabular}
}

\caption{Ablation experiments in the test set of THUMOS14.Performance evaluation on different Transformers decoder query}
\label{ablation_query}
\end{table}


==> table_tex/candidate_proposal.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{ccccccc}
\hline

Proposal Number & windows list  &0.3 &0.4 &0.5 &0.6&0.7 \\ \hline
608 & [5:5:65] & 62.5 & 56.6  & 48.7  & 39.7 & 28.4 \\ 
800 &  [2:5:62]   & 63.5 &57.6  & 49.8  & 40.5 & 29.4 \\ 
1218 &  [2:3:62]   & 64.6 & 58.5  & 50.0  & 40.4 & 28.1 \\ 
1726 &  [2:2:64]   & 65.2 & 59.1  & 50.8  & 41.0 & 28.8 \\ 
1225 & Fibonacci  & 65.3 & 59.3  & 50.8  & 40.1 & 28.5 \\ 

\hline
\end{tabular}
}

\caption{Ablation experiments in the test set of THUMOS14.Performance evaluation on 
different windows size list.}
\label{ablation candidate proposal number}
\end{table}

